Leveraging Prototypical Representations for Mitigating Social Bias without Demographic Information

Mitigating social biases typically requires identifying the social groups associated with each data sample. In this paper, we present DAFair, a novel approach to address social bias in language models. Unlike traditional methods that rely on explicit demographic labels, our approach does not require any such information. Instead, we leverage predefined prototypical demographic texts and incorporate a regularization term during the fine-tuning process to mitigate bias in the model's representations. Our empirical results across two tasks and two models demonstrate the effectiveness of our method compared to previous approaches that do not rely on labeled data. Moreover, with limited demographic-annotated data, our approach outperforms common debiasing approaches.

==> figures/bios-sizes.tex <==
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{emnlp2023-figures/bios_acc_sizes.png}
\caption{Accuracy}
\label{fig:bios_acc_sizes}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{emnlp2023-figures/bios_tpr_sizes.png}
\caption{TPR-GAP}
\label{fig:bios_tpr_sizes}
\end{subfigure}
\caption{Performance of bias mitigation methods on the occupation prediction task with varying sizes of labeled data for social attributes.}
\label{fig:dial_size}
\end{figure*}

==> figures/dial-sizes.tex <==
\begin{figure*}[ht]
\centering
\begin{subfigure}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{emnlp2023-figures/dial_acc_sizes.png}
\caption{Accuracy}
\label{fig:dial_acc_size}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{emnlp2023-figures/dial_tpr_sizes.png}
\caption{TPR-GAP}
\label{fig:dial_tpr_size}
\end{subfigure}
\caption{Performance of bias mitigation methods on the twitter sentiment task with varying sizes of labeled data for social attributes.}
\label{fig:bios_size}
\end{figure*}

==> tables/main-results-BIOS.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{table*}[!b]
\centering

\begin{tabular}{p{2.5cm}  cc  cc}
\toprule
 & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{DeBERTa} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Method & Acc $\uparrow$ & TPR-GAP $\downarrow$ & Acc $\uparrow$ & TPR-GAP $\downarrow$ \\
\midrule
Original & 83.43 & 14.66 & 83.42 & 14.60 \\
\midrule
JTT   & 81.34 & 14.86 & 81.01 & 13.86 \\
BLIND & 82.58 & 13.15 &  82.17 & 13.90\\
\methodName & 81.76 & 12.20 & 82.09 & 12.71 \\
\secondMethodName$^{*}$ & 80.22 & 11.87 & 80.16 & 11.16 \\
\bottomrule
\end{tabular}
\caption{Evaluation results on the test set for occupation prediction with BERT and DeBERTa as the encoders.}
\label{table:occupation}
\end{table*}


==> tables/main-results-DIAL.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{table*}[t]
\centering

\begin{tabular}{p{2.5cm}  cc  cc}
\toprule
 & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{DeBERTa} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Method & Acc $\uparrow$ & TPR-GAP $\downarrow$ & Acc $\uparrow$ & TPR-GAP $\downarrow$ \\
\midrule
Original & 79.18 & 24.54 & 78.36 & 29.62 \\
\midrule
JTT & 77.56 & 24.00 & 77.41 & 27.46 \\
BLIND & 76.36 & 22.54  & 77.20 & 27.32 \\
\methodName & 77.12 & 22.24 & 77.54 & 27.15 \\
\secondMethodName$^{*}$ & 76.86 & 19.93 & 75.80 & 25.46 \\
\bottomrule
\end{tabular}
\caption{Evaluation results on the test set for sentiment analysis with BERT and DeBERTa as the encoders.}
\label{table:sentiment}
\end{table*}


==> tables/main-results-deberta.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{table*}[!t]
\centering

\begin{tabular}{p{2.5cm}  cc  cc}
\toprule
 & \multicolumn{2}{c}{Occupation Prediction} & \multicolumn{2}{c}{Sentiment Analysis} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Method & Acc $\uparrow$ & TPR-GAP $\downarrow$ & Acc $\uparrow$ & TPR-GAP $\downarrow$ \\
\midrule
Original & $83.42\pm{\scriptstyle0.26}$ & $14.60\pm{\scriptstyle0.81}$ &
$78.36\pm{\scriptstyle0.93}$ & $29.62\pm{\scriptstyle1.58}$ \\
\midrule
JTT & $81.98\pm{\scriptstyle1.70}$ & $14.30\pm{\scriptstyle0.55}$ &
$77.41\pm{\scriptstyle1.76}$ & $28.06\pm{\scriptstyle2.03}$ \\
BLIND & $82.41\pm{\scriptstyle0.55}$ & $13.86\pm{\scriptstyle1.49}$ &
$77.20\pm{\scriptstyle1.22}$ & $27.32\pm{\scriptstyle2.84}$ \\
\methodName & \shadi{$82.15\pm{\scriptstyle0.32}$} & \shadi{$12.93\pm{\scriptstyle0.39}$} &
\shadi{$77.92\pm{\scriptstyle1.21}$} & \shadi{$26.24\pm{\scriptstyle1.61}$} \\
%\secondMethodName$^{*}$ & 76.86 & 19.93 & 75.80 & 25.46 \\
\bottomrule
\end{tabular}
\caption{Evaluation results for occupation prediction and sentiment analysis tasks with DeBERTa as the text encoders.}
\label{table:results-deberta}
\end{table*}


==> tables/main-results.tex <==
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{10pt}
\begin{table*}[t]
\centering

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{4cm}cccc}
\toprule
{} & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{DeBERTa} \\
\cline{2-5}
Method & Acc $\uparrow$ & TPR-GAP $\downarrow$ & Acc $\uparrow$ & TPR-GAP $\downarrow$ \\
\midrule
Finetuned & 83.43 & 14.66 & 83.42 & 14.60 \\
\hline
JTT & & & & \\
BLIND & 81.69 & 14.56 & 80.11 & 13.87  \\
\methodName & 81.76 & 12.29 & 82.09 & 12.71 \\
\bottomrule
\end{tabular}
\caption{Occupation Prediction}
\label{table:occupation}
\end{subtable}

\vspace{0.5cm}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{4cm}cccc}
\toprule
{} & \multicolumn{2}{c}{BERT} & \multicolumn{2}{c}{DeBERTa} \\
\cline{2-5}
Method & Acc $\uparrow$ & TPR-GAP $\downarrow$ & Acc $\uparrow$ & TPR-GAP $\downarrow$ \\
\midrule
Finetuned & 79.18 & 24.04 & 78.36 & 29.62 \\
\hline
JTT & 78.56 & 24.38 & 79.40 & 27.84 \\
BLIND & 78.46 & 21.64 & 78.05 & 26.27\\
\methodName & 76.07 & 21.88 & & \\
\bottomrule
\end{tabular}
\caption{Sentiment Analysis}
\label{table:sentiment}
\end{subtable}

\caption{Evaluation results on the test set with BERT and DeBERTa as the encoders.}
\label{table:main-bios}
\end{table*}

